TESS Hunt for Young and Maturing Exoplanets (THYME) X: a two-planet system in the 210 Myr MELANGE-5 Association

Young (<500 Myr) planets are critical to studying how planets form and evolve. Among these young planetary systems, multi-planet configurations are particularly useful as they provide a means to control for variables within a system. Here, we report the discovery and characterization of a young planetary system, TOI-1224. We show that the planet-host resides within a young population we denote as MELANGE-5 . By employing a range of age-dating methods -- isochrone fitting, lithium abundance analysis, gyrochronology, and Gaia excess variability -- we estimate the age of MELANGE-5 to be 210$\pm$27 Myr. MELANGE-5 is situated in close proximity to previously identified younger (80 -110 Myr) associations, Crius 221 and Theia 424/Volans-Carina, motivating further work to map out the group boundaries. In addition to a planet candidate detected by the TESS pipeline and alerted as a TESS Object of Interest, TOI-1224 b, we identify a second planet, TOI-1224 c, using custom search tools optimized for young stars (Notch and LOCoR). We find the planets are 2.10$\pm$0.09$R_\oplus$ and 2.88$\pm$0.10$R_\oplus$ and orbit their host star every 4.18 and 17.95 days, respectively. With their bright ($K$=9.1 mag), small ($R_{*}$=0.44R$_{\odot}$), and cool ($T_{eff}$ =3326K) host star, these planets represent excellent candidates for atmospheric characterization with JWST.

==> setup.tex <==
\usepackage{amsmath,amssymb}
\usepackage{epsfig}    
\usepackage{graphicx}    
\usepackage{lineno}
\usepackage{natbib}
\usepackage{bigints}
\usepackage[outdir=./]{epstopdf}

\usepackage[T1]{fontenc}
\pwifjournal\else
  \usepackage{microtype}
\fi

\pwifjournal\else
  \makeatletter
  \renewcommand\plotone[1]{%
    \centering \leavevmode \setlength{\plot@width}{0.95\linewidth}
    \includegraphics[width={\eps@scaling\plot@width}]{#1}%
  }%
  \makeatother
\fi


\makeatletter

\newcommand\@simpfx{http://simbad.u-strasbg.fr/simbad/sim-id?Ident=}

\newcommand\MakeObj[4][\@empty]{% [shortname]{ident}{url-escaped}{formalname}
  \pwifjournal%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\protect\object[#4]{##1}}%
  \else%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\href{\@simpfx #3}{##1}}%
  \fi%
  \expandafter\newcommand\csname pkgwobj@f#2\endcsname{#4}%
  \ifx\@empty#1%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#4}%
  \else%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#1}%
  \fi}%

\newcommand\MakeTrunc[2]{% {ident}{truncname}
  \expandafter\newcommand\csname pkgwobj@t#1\endcsname{#2}}%

\newcommand{\obj}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@s#1\endcsname}%
  \fi}
\newcommand{\objf}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@f#1\endcsname}%
  \fi}
\newcommand{\objt}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@t#1\endcsname}%
  \fi}

\makeatother


% Evil magic to patch natbib to only highlight the year paper refs, not the
% authors too; as seen in ApJ. From
% http://tex.stackexchange.com/questions/23227/.

\pwifjournal\else
  \usepackage{etoolbox}
  \makeatletter
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
         {\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
    {}{}
  \makeatother
\fi


% Object data

\providecommand{\eprint}[1]{\href{http://arxiv.org/abs/#1}{#1}}
\providecommand{\adsurl}[1]{\href{#1}{ADS}}
\newcommand{\mps}{m\,s$^{-1}$}
\providecommand{\icarus}{Icarus}
\newcommand{\vsini}{$v\sin{i_*}$}
\newcommand{\vdag}{(v)^\dagger}
\newcommand{\oxygen}{O$_2$}
\newcommand{\water}{H$_2$O}
\newcommand{\kepler}{{\it Kepler}}
\newcommand{\logg}{$log~g$ }
\newcommand{\metal}{[M/H]}
\newcommand{\um}{$\mu$m}
\newcommand{\fbol}{$F_{\mathrm{bol}}$}
\newcommand{\mbol}{$m_{\mathrm{bol}}$}
\newcommand{\Mbol}{$M_{\mathrm{bol}}$}
\newcommand{\rapsq}{$R_{ap}^2$}
\newcommand{\rchisq}{$\chi^2_{\nu}$}
\newcommand{\hipp}{{\it Hipparcos}}
\newcommand\teff{\ensuremath{T_\text{eff}}}
% utility

%\newcommand{\vdag}{(v)^\dagger}
%\newcommand{\oxygen}{O$_2$}
%\newcommand{\water}{H$_2$O}
%\newcommand{\kepler}{{\it Kepler}}
%\newcommand{\logg}{$log~g$ }
%\newcommand{\metal}{[M/H]}
%\newcommand{\um}{$\mu$m}
%\newcommand{\fbol}{$F_{\mathrm{bol}}$}
%\newcommand{\mbol}{$m_{\mathrm{bol}}$}
%\newcommand{\Mbol}{$M_{\mathrm{bol}}$}
%\newcommand{\rapsq}{$R_{ap}^2$}
%\newcommand{\rchisq}{$\chi^2_{\nu}$}
%\newcommand{\hipp}{{\it Hipparcos}}
%
%
%\newcommand\aafd{erg~s$^{-1}$~cm$^{-2}$~\AA$^{-1}$} % "AAngstrom flux density"
%\newcommand\amlt{$\alpha_{\rm MLT}$} % convective mixing length parameter
%\newcommand\apx{\ensuremath{\sim}}
%\newcommand\cgsflux{erg~s$^{-1}$~cm$^{-2}$}
%\newcommand\cgslum{erg~s$^{-1}$}
%\newcommand\chandra{\textit{Chandra}}
%\newcommand\citeeg[1]{\citep[\eg,][]{#1}}
%\newcommand\cps{ct~s$^{-1}$}
%\newcommand\dd{\ensuremath{\text{d}}}
%\newcommand\eg{\textit{e.g.}}
%\newcommand\etal{\textit{et~al.}}
%\newcommand\ewha{\ensuremath{\text{EW}(\ha)}}
%%\newcommand\fig[1]{Figure~\ref{f.#1}}
%\newcommand\ha{{\ensuremath{\text{H}\alpha}}}
%\newcommand\I{\mathcal{I}}
%\newcommand\ie{\textit{i.e.}}
\newcommand\kms{km~s$^{-1}$}
%\newcommand\ls{L$_\odot$}
%\newcommand\mj{M$_\text{J}$}
%\newcommand\ms{M$_\odot$}
%\newcommand\nupk{\ensuremath{\nu_\text{pk}}}
%\newcommand\percc{cm$^{-3}$}
%\newcommand\rcs{\ensuremath{\chi_r^2}}
%\newcommand\rj{R$_\text{J}$}
%\newcommand\sect[1]{Section~\ref{s.#1}}
%\newcommand\sherpa{\textsf{Sherpa}}
%\newcommand\sti{Stokes~$I$}
%\newcommand\stiv{Stokes~$I$ and~$V$}
%\newcommand\stv{Stokes~$V$}
%\newcommand\swift{\textit{Swift}}
%\newcommand\tb{\ensuremath{T_\text{b}}}
%\newcommand\tbl[1]{Table~\ref{t.#1}}
%\newcommand\teff{\ensuremath{T_\text{eff}}}
%\newcommand\todo[1]{\textcolor{red}{#1}}
%\newcommand\ujy{$\mu$Jy}
%\newcommand\ujybm{$\mu$Jy~bm$^{-1}$}
%\newcommand\uv{$u$\mbox{-}$v$}
%\newcommand\vsi{\ensuremath{v \sin i}}
%
%\newcommand\Lb{\ensuremath{L_\text{bol}}}
%\newcommand\Lh{\ensuremath{L_\ha}}
%\newcommand\Lr{\ensuremath{L_\text{R}}}
%\newcommand\sLr{\ensuremath{L_{\nu,\text{R}}}}
%\newcommand\Lu{\ensuremath{L_\text{UVW1}}}
%\newcommand\Lx{\ensuremath{L_\text{X}}}
%\newcommand\Lxf{\ensuremath{L_{\text{X},f}}}
%\newcommand\Lxq{\ensuremath{L_{\text{X},q}}}
%\newcommand\lb{\ensuremath{[\Lb]}}
%\newcommand\lh{\ensuremath{[\Lh]}}
%\newcommand\lr{\ensuremath{[\Lr]}}
%\newcommand\slr{\ensuremath{[\sLr]}}
%\newcommand\lu{\ensuremath{[\Lu]}}
%\newcommand\lx{\ensuremath{[\Lx]}}
%\newcommand\lxf{\ensuremath{[\Lxf]}}
%\newcommand\lxq{\ensuremath{[\Lxq]}}
%\newcommand\lhlb{\ensuremath{[\Lh/\Lb]}}
%\newcommand\lrlb{\ensuremath{[\Lr/\Lb]}}
%\newcommand\lulb{\ensuremath{[\Lu/\Lb]}}
%\newcommand\lxlb{\ensuremath{[\Lx/\Lb]}}
%\newcommand\lxflb{\ensuremath{[\Lxf/\Lb]}}
%\newcommand\lxqlb{\ensuremath{[\Lxq/\Lb]}}
%\newcommand\slrlb{\ensuremath{[\sLr/\Lb]}}
%\newcommand\slrlx{\ensuremath{[\sLr/\Lx]}}
%\newcommand\slrlxf{\ensuremath{[\sLr/\Lxf]}}
%\newcommand\slrlxq{\ensuremath{[\sLr/\Lxq]}}

